Real topological Hochschild homology and the Segal conjecture

We give a new proof, independent of Lin's theorem, of the Segal conjecture for the cyclic group of order two. The key input is a calculation, as a Hopf algebroid, of the Real topological Hochschild homology of $\mathbb{F}_2$. This determines the $\mathrm{E}_2$-page of the descent spectral sequence for the map $\mathrm{N}\mathbb{F}_2 \to \mathbb{F}_2$, where $\mathrm{N}\mathbb{F}_2$ is the $C_2$-equivariant Hill--Hopkins--Ravenel norm of $\mathbb{F}_2$. The $\mathrm{E}_2$-page represents a new upper bound on the $RO(C_2)$-graded homotopy of $\mathrm{N}\mathbb{F}_2$, from which the Segal conjecture is an immediate corollary.

==> differentials.tex <==
\section{Early computations}

\subsection{Low degree homotopy}

\begin{proposition} We have
	\[
	\pi_0 \mathrm{N}\mathbb{F}_2 =\mathbb{Z}/4
	\]
	\[
	\pi_\sigma\mathrm{N}\mathbb{F}_2 =
	\mathbb{Z}/4
	\]
The generator in $\pi_{\sigma}$ corresponds to $y_0$, and 
we have $ay_0 = 2$ and $ay_0^2 = \eta_{\sigma}$, the equivariant
Hopf element.
\end{proposition}

\subsection{Periodicity}

\begin{proposition} 
\end{proposition}

\subsection{A power operation and differential}

\begin{proposition} For $n>0$ we have
	\[
	d_2(y_n) = (ay_0) y_{n-1}^2.
	\]
\end{proposition}


\subsection{More low degree homotopy}


\begin{proposition} The first 
stems are given by:
	\begin{itemize}
	\item $\mathbb{Z}/4$
	\item $\mathbb{Z}/2 \{a^2y_1\}$
	\item $\mathbb{Z}/4 \{u^2y_0^2\}$
	\item $\mathbb{Z}/2\{a^4y_2\}
	\oplus \mathbb{Z}/2\{au^2y_0y_1\}$
	\item $\mathbb{Z}/2\{u^4y_0^4\}$
	\item $\mathbb{Z}/2\{au^4y_0^3y_1\}$
	\item $\mathbb{Z}/2\{u^6y_0^6\} \oplus
	\mathbb{Z}/4\{u^4y_1^2\}$
	\end{itemize}

\end{proposition}

\begin{proof} In low degrees the $E_2$-term of the spectral
sequence looks like:

Here $(ay_0)^{\varepsilon}(u^2y_0^2)$ and its powers 
are permanent cycles by
as is $a^2y_1$ for degree reasons. The only possible differential
on $a^4y_2$ is a $d_2$, but we have
	\[
	d_2(a^4y_2) = a^4(ay_0y_1^2) = 0
	\]
so $a^4y_2$ is a permanent cycle. There is a differential
	\[
	d_2(u^4y_0^2y_1) = au^4 y_0^5
	\]
which takes care of stem 4. There is no
$d_2$-differential on $u^4y_1^2$ because it is a square,
it is too low to be the target of a differential,
and there is no room for further differentials, so it survives
along with the potential target in stem 5. 

This is good enough to pin down through stem 5, and
stem 6 is almost there but we have to rule out a few
more differentials coming in...
\end{proof}

I think we might be able to argue that $u^2y_0^2$
is nonnilpotent... since it ought to correspond to
a transfer. That should help things...

Actually: we can probably identify transfer classes by
figuring out the Hurewicz map... they'll basically be precisely
the nonnilpotent things, and so must be detected by Hurewicz.








